PoE-Fuse: Precision-Weighted Expert Fusion for Bi-Temporal Change Understanding

Bi-temporal change understanding, which localizes and characterizes what changed between two satellite images, is central to disaster response and environmental monitoring, spanning change detection, building localization, and damage assessment. Strong vision-language models address these tasks, but adapting them typically requires full fine-tuning or reinforcement learning, which is costly and unstable. We propose PoE-Fuse, a parameter-efficient framework that instead composes frozen foundation experts for geometry, grounding, and language, resampling their features onto a shared spatial grid and training only a lightweight fusion trunk. PoE-Fuse treats the aligned features as Gaussian observations of a latent scene state and fuses them by learned per-cell precision. This product-of-experts estimator strictly generalizes uniform summation and scalar gating, and extends to change fields by composing the precisions of the two timestamps. A single shared trunk solves the three tasks at once, reaching a mean F1 of 59.2%, compared with 40.7% for an instruction-tuned temporal vision-language assistant, and surpassing dedicated change-detection models retrained under the same protocol and training budget.

==> tex/sections/supp_titlepage.tex <==
% Supplementary title page (shared by standalone supp.tex and the optional
% combined-review build at the end of main.tex).
\begin{center}
  {\Large\bfseries PoE-Fuse: Precision-Weighted Expert Fusion\\ for Bi-Temporal Change Understanding\par}
  \vspace{4pt}
  {\Large\bfseries Supplementary Material\par}
  \vspace{22pt}
  Haruki Watase$^{\star}$, Shunya Nagashima$^{\star}$, and Takayuki Nishimura\par
  \vspace{8pt}
  Neurogica Inc., Tokyo, Japan\par
  \texttt{\{haruki.watase,shunya.nagashima,takayuki.nishimura\}@neurogica.com}\par
  \vspace{6pt}
  {\small $^{\star}$Equal contribution.\par}
\end{center}
\vspace{18pt}

